Evolution of Voronoi based Fuzzy Recurrent Controllers

A fuzzy controller is usually designed by formulating the knowledge of a human expert into a set of linguistic variables and fuzzy rules. Among the most successful methods to automate the fuzzy controllers development process are evolutionary algorithms. In this work, we propose the Recurrent Fuzzy Voronoi (RFV) model, a representation for recurrent fuzzy systems. It is an extension of the FV model proposed by Kavka and Schoenauer that extends the application domain to include temporal problems. The FV model is a representation for fuzzy controllers based on Voronoi diagrams that can represent fuzzy systems with synergistic rules, fulfilling the $\epsilon$-completeness property and providing a simple way to introduce a priory knowledge. In the proposed representation, the temporal relations are embedded by including internal units that provide feedback by connecting outputs to inputs. These internal units act as memory elements. In the RFV model, the semantic of the internal units can be specified together with the a priori rules. The geometric interpretation of the rules allows the use of geometric variational operators during the evolution. The representation and the algorithms are validated in two problems in the area of system identification and evolutionary robotics.

==> Figures/rfv.tex <==
% PSTricks TeX macro
% Title: /home/ckavka/Papers/Cacic2004/Figuras/modelo.fig
% Creator: Dia v0.94
% CreationDate: Mon Jan  3 20:59:12 2005
% For: ckavka
% \usepackage{pstricks}
% The following commands are not supported in PSTricks at present
% We define them conditionally, so when they are implemented,
% this pstricks file will use them.
\ifx\setlinejoinmode\undefined
  \newcommand{\setlinejoinmode}[1]{}
\fi
\ifx\setlinecaps\undefined
  \newcommand{\setlinecaps}[1]{}
\fi
% This way define your own fonts mapping (for example with ifthen)
\ifx\setfont\undefined
  \newcommand{\setfont}[2]{}
\fi
\pspicture(0.746125,-14.493875)(14.303375,-4.556125)
\scalebox{1.000000 -1.000000}{
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\newrgbcolor{diafillcolor}{1.000000 1.000000 1.000000}
\psset{fillcolor=diafillcolor}
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(6.000750,6.191250)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(6.000750,7.334250)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(6.000750,11.525250)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon(5.334000,5.334000)(5.334000,12.382500)(6.667500,12.382500)(6.667500,5.334000)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(9.048750,6.191250)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(9.048750,7.334250)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(9.048750,11.525250)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon(8.382000,5.334000)(8.382000,12.382500)(9.715500,12.382500)(9.715500,5.334000)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(2.952750,5.334000)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(2.952750,6.381750)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(2.952750,7.905750)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(2.952750,9.715500)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(2.952750,10.763250)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(2.952750,12.287250)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon(2.286000,4.572000)(2.286000,8.763000)(3.619500,8.763000)(3.619500,4.572000)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon(2.286000,8.953500)(2.286000,13.144500)(3.619500,13.144500)(3.619500,8.953500)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(12.096750,5.334000)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(12.096750,6.381750)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(12.096750,7.905750)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(12.096750,9.715500)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(12.096750,10.763250)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psellipse(12.096750,12.287250)(0.425450,0.425450)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon(11.430000,4.572000)(11.430000,8.763000)(12.763500,8.763000)(12.763500,4.572000)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon(11.430000,8.953500)(11.430000,13.144500)(12.763500,13.144500)(12.763500,8.953500)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,5.334000)(5.524500,6.191250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,6.381750)(5.524500,7.334250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,5.334000)(5.524500,7.334250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,5.334000)(5.524500,11.620500)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,6.381750)(5.524500,6.191250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,6.381750)(5.524500,11.620500)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,7.905750)(5.524500,6.191250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,7.905750)(5.524500,7.334250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,7.905750)(5.524500,11.620500)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,9.715500)(5.524500,6.191250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,9.715500)(5.524500,7.334250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,9.715500)(5.524500,11.620500)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,10.763250)(5.524500,6.191250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,10.763250)(5.524500,7.334250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,10.763250)(5.524500,11.620500)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,12.287250)(5.524500,6.191250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,12.287250)(5.524500,7.334250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(3.429000,12.287250)(5.524500,11.620500)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(6.477000,6.191250)(8.302625,6.191250)
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon*(8.302625,6.254750)(8.556625,6.191250)(8.302625,6.127750)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(6.477000,7.334250)(8.302625,7.334250)
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon*(8.302625,7.397750)(8.556625,7.334250)(8.302625,7.270750)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(6.477000,11.525250)(8.302625,11.525250)
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon*(8.302625,11.588750)(8.556625,11.525250)(8.302625,11.461750)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,6.191250)(11.620500,5.334000)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,6.191250)(11.620500,6.381750)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,6.191250)(11.620500,7.905750)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,6.191250)(11.620500,9.715500)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,6.191250)(11.620500,10.763250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,6.191250)(11.620500,12.287250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,7.334250)(11.620500,5.334000)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,7.334250)(11.620500,6.381750)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,7.334250)(11.620500,7.905750)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,7.334250)(11.620500,9.715500)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,7.334250)(11.620500,10.763250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,7.334250)(11.620500,12.287250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,11.525250)(11.620500,5.334000)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,11.525250)(11.620500,6.381750)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,11.525250)(11.620500,7.905750)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,11.525250)(11.620500,10.763250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,11.525250)(11.620500,12.287250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(0.762000,5.334000)(2.206625,5.334000)
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon*(2.206625,5.397500)(2.460625,5.334000)(2.206625,5.270500)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(0.762000,6.381750)(2.206625,6.381750)
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon*(2.206625,6.445250)(2.460625,6.381750)(2.206625,6.318250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(0.762000,7.905750)(2.206625,7.905750)
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon*(2.206625,7.969250)(2.460625,7.905750)(2.206625,7.842250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(1.333500,9.715500)(2.206625,9.715500)
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon*(2.206625,9.779000)(2.460625,9.715500)(2.206625,9.652000)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(1.333500,10.763250)(2.206625,10.763250)
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon*(2.206625,10.826750)(2.460625,10.763250)(2.206625,10.699750)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(1.333500,12.287250)(2.206625,12.287250)
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon*(2.206625,12.350750)(2.460625,12.287250)(2.206625,12.223750)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(12.573000,5.334000)(14.017625,5.334000)
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon*(14.017625,5.397500)(14.271625,5.334000)(14.017625,5.270500)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(12.573000,6.381750)(14.017625,6.381750)
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon*(14.017625,6.445250)(14.271625,6.381750)(14.017625,6.318250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(12.573000,7.905750)(14.017625,7.905750)
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon*(14.017625,7.969250)(14.271625,7.905750)(14.017625,7.842250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(12.573000,10.763250)(13.716000,10.763250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(12.573000,12.287250)(13.716000,12.287250)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(9.525000,11.525250)(11.620500,9.715500)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon(6.858000,13.335000)(6.858000,14.478000)(8.191500,14.478000)(8.191500,13.335000)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(12.573000,9.715500)(13.716000,9.715500)(13.716000,13.906500)(8.461375,13.906500)
\setlinejoinmode{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\pspolygon*(8.461375,13.843000)(8.207375,13.906500)(8.461375,13.970000)
\psset{linewidth=0.031750}
\psset{linestyle=solid}
\psset{linestyle=solid}
\setlinejoinmode{0}
\setlinecaps{0}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\psline(6.858000,13.906500)(1.333500,13.906500)(1.333500,9.715500)
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](2.762250,6.477000){\scalebox{1 -1}{$x_2$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](2.762250,9.810750){\scalebox{1 -1}{$y_1$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](2.762250,8.001000){\scalebox{1 -1}{$x_l$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](2.762250,10.858500){\scalebox{1 -1}{$y_2$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](2.762250,12.382500){\scalebox{1 -1}{$y_r$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](11.906250,5.524500){\scalebox{1 -1}{$v_1$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](11.906250,6.572250){\scalebox{1 -1}{$v_2$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](11.906250,8.096250){\scalebox{1 -1}{$v_m$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](11.906250,10.953750){\scalebox{1 -1}{$y_2$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](11.906250,12.477750){\scalebox{1 -1}{$y_r$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](11.906250,9.906000){\scalebox{1 -1}{$y_1$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](2.762250,5.524500){\scalebox{1 -1}{$x_1$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](7.239000,14.001750){\scalebox{1 -1}{$z^{-1}$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](8.858250,11.620500){\scalebox{1 -1}{$R_ega$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](8.763000,7.429500){\scalebox{1 -1}{$R_2$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](8.763000,6.286500){\scalebox{1 -1}{$R_1$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](5.810250,6.286500){\scalebox{1 -1}{$S_1$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](5.810250,7.429500){\scalebox{1 -1}{$S_2$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](5.810250,11.620500){\scalebox{1 -1}{$S_ega$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](5.715000,9.429750){\scalebox{1 -1}{$ots$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](8.763000,9.429750){\scalebox{1 -1}{$ots$}}
\setfont{AvantGarde-Book}{0.540833}
\newrgbcolor{dialinecolor}{0.000000 0.000000 0.000000}
\psset{linecolor=dialinecolor}
\rput[l](7.143750,9.429750){\scalebox{1 -1}{$ots$}}
}\endpspicture
